SketchMetaFace: A Learning-based Sketching Interface for High-fidelity 3D Character Face Modeling

Modeling 3D avatars benefits various application scenarios such as AR/VR, gaming, and filming. Character faces contribute significant diversity and vividity as a vital component of avatars. However, building 3D character face models usually requires a heavy workload with commercial tools, even for experienced artists. Various existing sketch-based tools fail to support amateurs in modeling diverse facial shapes and rich geometric details. In this paper, we present SketchMetaFace - a sketching system targeting amateur users to model high-fidelity 3D faces in minutes. We carefully design both the user interface and the underlying algorithm. First, curvature-aware strokes are adopted to better support the controllability of carving facial details. Second, considering the key problem of mapping a 2D sketch map to a 3D model, we develop a novel learning-based method termed "Implicit and Depth Guided Mesh Modeling" (IDGMM). It fuses the advantages of mesh, implicit, and depth representations to achieve high-quality results with high efficiency. In addition, to further support usability, we present a coarse-to-fine 2D sketching interface design and a data-driven stroke suggestion tool. User studies demonstrate the superiority of our system over existing modeling tools in terms of the ease to use and visual quality of results. Experimental analyses also show that IDGMM reaches a better trade-off between accuracy and efficiency. SketchMetaFace is available at https://zhongjinluo.github.io/SketchMetaFace/.

==> figure/fig_algo_compare_merge.tex <==
\begin{figure}[htb]
\centering
\hspace{-3mm}\begin{minipage}[t]{0.425\textwidth}
  \centering
  \includegraphics[width=0.88\linewidth]{image/base_level_1000.pdf}
  \caption{Qualitative comparisons on part-separated mesh inference from an input sketch (a). (b) The results of our part-separated PIFu. (c) The results of Pixel2Mesh. (d) The results of retrieval. }
  \label{fig:base_level}
\end{minipage}
\hspace{3mm}\begin{minipage}[t]{0.49\textwidth}
  \centering
  \includegraphics[width=1.\linewidth]{image/algo_compare_1000.pdf}
 \caption{Qualitative comparisons of our IDGMM with four existing methods for Sketch2Mesh inference.}
  \label{fig:algo_compare}
\end{minipage}
\end{figure}

==> figure/fig_gallery_u_system_c.tex <==
\begin{figure}[htbp]
\centering
\begin{minipage}[t]{0.51\textwidth}
  \centering
  \includegraphics[width=.98\linewidth]{image/gallery_usability2.pdf}
  \caption{A gallery of the 3D face models created by the novice users.}
  \label{fig:gallery_user}
\end{minipage}
\begin{minipage}[t]{0.48\textwidth}
  \centering
  \includegraphics[width=.98\linewidth]{image/system_compare_2.pdf}
  \caption{Comparison of our system against two existing systems. Some representative examples are shown. The results in each row were created by the same user given a reference in (a).}
  \label{fig:system_compare}
\end{minipage}
\end{figure}

==> figure/fig_gallery_user.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=.98 \linewidth]{image/gallery_usability2.pdf}
  \caption{A gallery of the 3D face models created by the novice users.}
  \label{fig:gallery_user}
\end{figure}

==> figure/fig_stroke_ablation_limitation.tex <==
\begin{figure}[htbp]
\centering
\begin{minipage}[t]{0.63\textwidth}
  \centering
  \includegraphics[width=.96 \linewidth]{image/rgb_2.pdf}
  \caption{Ablation study on without/with curvature-aware strokes.}
  \label{fig:black_stroke}
\end{minipage}
\begin{minipage}[t]{0.35\textwidth}
  \centering
  \includegraphics[width=.96 \linewidth]{image/limitation_3.pdf}
  \caption{Limitations of our system. %Our system also suffers from limitations when 1) modeling facial components or details with complex depth changes; 2) strokes are placed too densely.
  }
  \label{fig:limitation}
\end{minipage}
\end{figure}

==> figure/fig_stroke_depth_width.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=.78 \linewidth]{image/stroke_depth_width2_1.pdf}
  \caption{An illustration of curvature-aware strokes: valley strokes in green and ridge strokes in red. By tuning the width and intensity of the curvature-aware strokes, users can precisely express their design ideas on surface details.}
  \label{fig:stroke_depth_width}
\end{figure}

==> figure/fig_suggestion_coarse.tex <==
\begin{figure}[htbp]
\centering
\begin{minipage}[t]{0.45\textwidth}
  \centering
  \includegraphics[width=.95\textwidth]{image/sugg_2000.pdf}
  \caption{An illustration of our stroke suggestion component. Soon after users specify the style, target region, and facial components to be modeled, the stroke suggestion component retrieves the relevant curvature-aware strokes. Users may also manipulate the layout for the retrieved strokes through dragging and scaling. }
  \label{fig:suggestion}
\end{minipage}

\hspace{2mm}\begin{minipage}[t]{0.52\textwidth}
  \centering
  \includegraphics[width=1.\textwidth]{image/coarse_modeling.pdf}
  \caption{The architecture of our part-separated coarse modeling of a 3D face with an outline sketch input $S_r$. It first generates three parts of a face region and two ears using \emph{PIFu}, and then assembles and merges them to obtain a coarse model $M_c$.
  }
  \label{fig:pipeline_coarse}
\end{minipage}
\end{figure}

==> figure/fig_zb.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=.98 \linewidth]{image/zb_3.pdf}
  \caption{A simple study to compare our system with ZBrush. For each example, the left model was created by our system. An experienced artist was recruited and asked to duplicate the left model % given the left model and asked to duplicate
  given a time limit of 10 minutes. %within 10 minutes restriction. 
  The created models are shown on the right of each example. }
  \label{fig:zb}
\end{figure}

==> figure/fig_zb_table.tex <==
\begin{figure}[htbp]
\centering
\begin{minipage}[b]{0.40\linewidth}
  \centering
  \includegraphics[width=.98\linewidth]{image/zb_3.pdf}
  \caption{A simple study to compare our system with ZBrush. For each example, the left model was created by our system. An experienced artist was recruited and asked to duplicate the left model % given the left model and asked to duplicate
  given a time limit of 10 minutes. %within 10 minutes restriction. 
  The created models are shown on the right of each example. }
  \label{fig:zb}
\end{minipage}
\begin{minipage}[b]{0.56\linewidth}
  \centering
  \begin{tabular}{l||c|c|c}
	& IoU $\uparrow$   & Chamfer-$L_2$ ($\times 10^2)$ $\downarrow$  & Normal-Consis. $\uparrow$ \\ \hline \hline 
	3D-R2N2 & 0.858 & 0.149 & 0.929 \\  %\hline
	Pixel2Mesh & 0.882 & 0.123 & 0.937 \\ 
	DeepSDF & 0.894 & 0.117 & 0.949 \\ 
% 			SAniHead & 0.831 & 0.210 & 0.921 \\
	PIFuHD & 0.911 & 0.103 & \textbf{0.956} \\
	Ours & \textbf{0.915} & \textbf{0.099} & 0.955 \\
    \end{tabular}
    \captionof{table}{Quantitative comparison with our proposed IDGMM with four existing methods for Sketch2Mesh inference. We adopt four metrics of IoU, Chamfer-$L_2$, normal consistency, and proximity to evaluate the results.}
    \label{tab:quant_fine}
\end{minipage}
\end{figure}

==> section/store.tex <==


%Rhowever, in real scenarios, we usually want a character face with diverse styles, for example, a human face with a pig nose (the Monk Pig in Fig.~\ref{}). 2) it is hard to model vivid surface details; however, a character's face is usually full of geometric details (the Thanos in Fig.~\ref{}).

%Among them, DeepSketch2Face~\cite{han2017deepsketch2face} is the . It proposes the first deep learning-based sketching system for modeling 3D caricatures or real faces. The key technique is a learning-based method that maps 2D sketch drawings to parametric morphable model space. Limited to the representation capability of the parametric model, DeepSketch2Face suffers from two significant limitations: 1) it can only model fixed-style faces (i.e., topological consistent with a template mesh); however, in real scenarios, we usually want a character face with diverse styles, for example, a human face with a pig nose (the Monk Pig in Fig.~\ref{}). 2) it is hard to model vivid surface details; however, a character's face is usually full of geometric details (the Thanos in Fig.~\ref{}).

%In contrast, in MMORPGs, social media, and virtual live streaming, amateur users expect to customize their avatars in arbitrary styles within a few minutes. As most amateur users lack expertise in 3D modeling and easily get frustrated, the ``formal'' 3D content generation pipeline may not be applicable. Moreover, compared with modeling virtual avatars of real-world humans, customizing avatars with arbitrary styles, e.g., caricature-like, animal-like, cartoon-like, is exceptionally challenging for novice users as the desired shapes are with more diversified geometry and meticulous surface details.

%To address the above issues, this paper proposed a powerful sketch modeling system for freestyle and high-fidelity 3D faces, targeting at the following challenges in sketch based modeling: 
%\noindent \textit{Accuracy}
%Thus, in this paper, our objective is to design a more powerful sketching system for freestyle and high-fidelity face modeling. From the users' perspective, the system needs to satisfy the following requirements: 1) \textit{Accuracy} of the output - the resulted 3D shape needs to resemble well what the users' drawing; 2) \textit{Instance} of the response - during the sketching procedure, the system can generate results responsively; 3) \textit{Usability} of the system - amateur users can learn how to use the system in a short time. We thoroughly considered these criteria and carefully designed both the interface and algorithm:

%\begin{itemize}
% \begin{enumerate}

%Unlike existing commercialized 3D modeling software that is much too complicated for invoice users, sketch modeling provides a more casual and agile way to design 3D shapes. Following the ground-breaking work of Igarashi et al.~\cite{igarashi1999teddy}, extensive research has been conducted that allows users without expertise in 3D modeling to create 3D content with free-hand sketches. Recent research on sketch modeling can be roughly divided into two streams, i.g., free form surface modeling and class-specific shape modeling. In sketch modeling systems for freeform surfaces, users can design 3D shapes by specifying contours and surface features explicitly with mono-typed or semantic sketch strokes. However, without proper prior knowledge of the intended 3D shape, these systems usually require users to make extensive specifications to generate desired shapes. In contrast, class-specific sketch modeling systems allow users to reconstruct visually plausible 3D shapes within a few strokes through retrieval or interpolation within the database. Nevertheless, these systems fall short in controlling the appearances of the generated shapes, and the generated shapes are bounded within a specific category.

%Closer to our work, Deepsketch2face proposed a novel sketch-based modeling system that allows users to customize caricature head models with free-hand sketches from scratch. However, Deepsketch2face suffers from two significant drawbacks, ambiguous sketch strokes and non-expressive back-end models, both hinder users from creating novel articulated avatars with more diversified appearances(e.g., orcs, goblins that are prevalent in video games and virtual live streaming):

%Let us first look back at the interactive 3D modeling scheme proposed in Deepsketch2face. Users may define the shape of the caricature heads by sketching sparse contour lines and further refine the sketching model with gesture-based refinement. Notably, for the sake of the system's intuitiveness, Deepsketch2face only allowed users to sketch with one type of sketch stroke. We argue that such design may hinder the users from freely specifying their desired avatar shapes due to the ambiguity of the mono-typed sketch strokes. Secondly, as the sketching shape generation module for Deepsektch2face depends solely on a parametric morphable model, it cannot produce novel geometries or surface wrinkle details reflecting the appearances of the sketch input.

%In this paper, to address the issues mentioned above, we firstly proposed a novel sketch-based modeling interface that assists users in creating the high-fidelity 3D face of arbitrary styles from scratch. In terms of sketching ambiguity, we introduce curvature-aware strokes to empower users to carve more detailed 3D avatars via freehand sketches. Compared with Deepsketch2face, which adopts mono-type sketch strokes, the curvature-aware strokes can significantly reduce the ambiguity in defining the contours and details of the shape. Moreover, to alleviate users' cognitive load when sketching with curvature-aware strokes, we proposed a dedicated designed method that generates curvature-aware sketch strokes from raw freehand mono-typed sketches. The generated strokes may serve as an intermediate result and guidance for further sketching. Apart from the intuitive user interface, we proposed a novel back-end model that produces high-quality 3D faces of arbitrary style from curvature-aware sketch strokes in real-time.
%Creating visually plausible virtual avatars is a prolonged research topic in visual computing and human-computer interaction, aimed at satisfying the demands of different usage scenarios. For ``high-end'' applications like filming, experienced artists may spend months formally sculpting high-fidelity 3D avatars with vivid surface details using powerful commercialized 3D modeling tools, e.g., ZBrush, MAYA, and 3D MAX.
%To allow amateur users being able to design 3D shapes in their mind,

%Thanks to the better understanding of shape and free-hand sketches provided by recent recent progress
%With the recent progress in deep-learning, smarter modeling tools have been proposed, 

%Due to their powerful inference ability, deep learning techniques are recently adopted for sketch understanding and support the development of smarter modeling tools~\cite{han2017deepsketch2face,li2018robust,li2020sketch2cad,du2020sanihead,du2020learning,luo2021simpmodeling}.


%\noindent \textit{\textbf{Accuracy}.} a) From interface view, to allow users to easily express surface details, we newly defined a curvature-aware stroke. More specifically, we use different strokes to represent ridge and valley lines which are also assigned tunable depth and width attributes. This kind of sketching also eases the learning procedure from a 2D drawings to geometric details. b) From algorithm view, although there already has many existing works~\cite{choy20163d,wang2018pixel2mesh,groueix2018papier,mescheder2019occupancy,park2019deepsdf,chen2019learning,saito2019pifu,saito2020pifuhd} can map a 2D image (sketch can also be treated as an image) to a 3D shape, it still remains challenges to model a watertight mesh with details. Among existing works, applying a pix2pix~\cite{isola2017image} model to translate the input sketch to a depth map can better infer details and its result can also well-matches the input, while it is difficult to create a watertight mesh from depth maps. Another method which can also well-resemble the input is pixel-aligned implicit function (PIFu)~\cite{saito2019pifu}. However, the used implicit representation makes it difficult to model high-frequency details. We then propose a novel approach to combine depth and implicit representations and take both of their advantages, which is named Implicit and Depth Guided Mesh Modeling (IDGMM).
